Robust Convergence of Parareal Algorithms with Arbitrarily High-order Fine Propagators

The aim of this paper is to analyze the robust convergence of a class of parareal algorithms for solving parabolic problems. The coarse propagator is fixed to the backward Euler method and the fine propagator is a high-order single step integrator. Under some conditions on the fine propagator, we show that there exists some critical $J_*$ such that the parareal solver converges linearly with a convergence rate near $0.3$, provided that the ratio between the coarse time step and fine time step named $J$ satisfies $J \ge J_*$. The convergence is robust even if the problem data is nonsmooth and incompatible with boundary conditions. The qualified methods include all absolutely stable single step methods, whose stability function satisfies $|r(-\infty)|<1$, and hence the fine propagator could be arbitrarily high-order. Moreover, we examine some popular high-order single step methods, e.g., two-, three- and four-stage Lobatto IIIC methods, and verify that the corresponding parareal algorithms converge linearly with a factor $0.31$ and the threshold for these cases is $J_* = 2$. Intensive numerical examples are presented to support and complete our theoretical predictions.

==> Parareal-Single (2)/tmp_parareal_abstract.tex <==
\begin{abstract}
The aim of this paper is to analyze the robust convergence of a class of parareal algorithms for solving
parabolic problems. The coarse propagator is fixed to the backward Euler method
and the fine propagator is a high-order single step integrator.
Under some conditions on the fine propagator,
we show that there exists some critical $J_*$ such
that the parareal solver converges linearly with a convergence rate near $0.3$,
provided that the ratio between the coarse time step and fine
time step named $J$ satisfies $J \ge J_*$.
The convergence is robust even if the problem data is nonsmooth and incompatible with boundary conditions. The qualified methods include all absolutely stable single step methods,
%all absolutely stable Runge--Kutta integrators
whose stability function satisfies $|r(-\infty)|<1$,
and hence the fine propagator could be arbitrarily high-order. Moreover, we examine some popular high-order single step methods, e.g., two-, three- and four-stage Lobatto IIIC methods,
and verify that the corresponding parareal algorithms converge linearly with a factor $0.31$ and the threshold for these cases is $J_* = 2$.
Intensive numerical examples are presented to support and complete our theoretical predictions.
\end{abstract}



\begin{keywords}
parareal algorithm, parabolic problems, arbitrarily high-order,
single step integrator, convergence factor
\end{keywords}

\begin{AMS}
Primary 65M12, 65M60; Secondary 65L06
\end{AMS}


==> Parareal-Single (2)/tmp_parareal_header.tex <==
\title{Robust Convergence of Parareal Algorithms with Arbitrarily High-order Fine Propagators
\thanks{\funding{The work of J.\ Yang is supported by National Natural Science Foundation of China (NSFC) Grant No. 11871264%, Natural Science Foundation of Guangdong Province (2018A0303130123), and NSFC/Hong Kong RRC Joint Research Scheme (NFSC/RGC 11961160718),
and the research of Z.\ Yuan and Z.\ Zhou is partially supported by Hong Kong RGC grant (No. 15304420).}}}








\author{Jiang Yang\thanks{Department of Mathematics \& SUSTech International Center for Mathematics,
Southern University of Science and Technology, Shenzhen 518055, China.
(\texttt{yangj7sustech.edu.cn})}
\and Zhaoming Yuan\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong. Department of Mathematics \& SUSTech International Center for Mathematics,
Southern University of Science and Technology, Shenzhen 518055, China.
(\texttt{zhaoming.yuan@connect.polyu.hk})}
\and Zhi Zhou\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Kowloon, Hong Kong.
(\texttt{zhizhou@polyu.edu.hk, zhizhou0125@gmail.com})}}
\date{\today}





% Custom SIAM macro to insert headers
\headers{Parareal Algorithms with Arbitrarily High-order Fine Propagators}{Jiang Yang, Zhaoming Yuan and Zhi Zhou}

